AutoSearch: Adaptive Search Depth for Efficient Agentic RAG via Reinforcement Learning

Agentic retrieval-augmented generation (RAG) systems enable large language models (LLMs) to solve complex tasks through multi-step interaction with external retrieval tools. However, such multi-step interaction often involves redundant search steps, incurring substantial computational cost and latency. Prior work limits search depth (i.e., the number of search steps) to reduce cost, but this often leads to underexploration of complex questions. To address this, we first investigate how search depth affects accuracy and find a minimal sufficient search depth that defines an accuracy-efficiency trade-off, jointly determined by question complexity and the agent's capability. Furthermore, we propose AutoSearch, a reinforcement learning (RL) framework that evaluates each search step via self-generated intermediate answers. By a self-answering mechanism, AutoSearch identifies the minimal sufficient search depth and promotes efficient search by rewarding its attainment while penalizing over-searching. In addition, reward mechanisms are introduced to stabilize search behavior and improve answer quality on complex questions. Extensive experiments on multiple benchmarks show that AutoSearch achieves a superior accuracy-efficiency trade-off, alleviating over-searching while preserving search quality.

==> latex/rebuttal.tex <==



Reviewer1 
Summary Of Weaknesses:
1. The judgement of outcome reward and the measurement of "capability-aware optimal search depth" () relies strictly on EM with the ground truth, unlike the final accuracy during testing which is judged on both EM and F1. EM might be too strict for some questions that requires long form, complex answers, or answering with certain style of output (such as answering a person's full name vs. only first name + last name). A semantic based method could be more appropriate.
2. The method generates an intermediate answer at each retrieval step to estimate optimal search depth. This implies extra token and time consumption per step during training. Although the authors include analysis on Search Time and Token Length in Section 5.4 and Figure 6, it is unclear that whether these analysis included the overhead during training. An analysis of the overhead (latency and/or percetnage of extra time comsumption) of the validation methods during training will be helpful.
3. The formulas of computing rewards include several fixed numbers (such as -0.05, 0.1, -0.5 in Formula 1). However, there seems to be no explanation on how do these numbers are come up. If these numbers can be considered as hyperparameters of the method, an extra analysis on this is preferred.
Comments Suggestions And Typos:
This is not a weakness but more of a question. Case 4 and 5 for comparing HIPRAG and AutoSearch show that these two method use the same output formatting. However, in HIPRAG[1], the format is actually different than the format shown in the Case 4 and 5 with extra [object Object] and [object Object] tags. Can the author explain this discrepancy?
[1] Wu et al. 2025. HiPRAG: Hierarchical Process Rewards for Efficient Agentic Retrieval Augmented Generation. arXiv preprint arXiv:2510.07794.









\begin{table*}[t]
\centering
\caption{ \textbf{(Main Results)} EM, F1, Search Depth and Search Efficiency Comparison Across Methods.}
\label{tab:qa_main_metrics}
\small
\setlength{\tabcolsep}{4.0 pt}
\renewcommand{\arraystretch}{1.0}

% 不使用 resizebox，除非必要
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l *{14}{c}}
\toprule
\multirow{3}{*}{\textbf{Method}} &
\multicolumn{6}{c}{\textbf{General QA}} &
\multicolumn{8}{c}{\textbf{Multi-Hop QA}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-15}
&
\multicolumn{2}{c}{\textbf{NQ}} &
\multicolumn{2}{c}{\textbf{TriviaQA}} &
\multicolumn{2}{c}{\textbf{PopQA}} &
\multicolumn{2}{c}{\textbf{HotpotQA}} &
\multicolumn{2}{c}{\textbf{2Wiki}} &
\multicolumn{2}{c}{\textbf{Bamboogle}} &
\multicolumn{2}{c}{\textbf{Avg}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15}
& 
\scriptsize \textbf{EM $\uparrow$} & \scriptsize \textbf{F1 $\uparrow$} &
\scriptsize \textbf{EM $\uparrow$} & \scriptsize \textbf{F1 $\uparrow$} &
\scriptsize \textbf{EM $\uparrow$} & \scriptsize \textbf{F1 $\uparrow$} &
\scriptsize \textbf{EM $\uparrow$} & \scriptsize \textbf{F1 $\uparrow$} &
\scriptsize \textbf{EM $\uparrow$} & \scriptsize \textbf{F1 $\uparrow$} &
\scriptsize \textbf{EM $\uparrow$} & \scriptsize \textbf{F1 $\uparrow$} &
\scriptsize \textbf{EM $\uparrow$} & \scriptsize \textbf{F1 $\uparrow$} \\

\midrule

% === Qwen2.5-3B Results ===


\rowcolor{green!10}
\multicolumn{15}{l}{\textit{\textbf{Base model: Qwen2.5-3b-Base/Instruct}}} \\

Search-R1-base           &\underline{36.0}& \underline{44.9}& 51.3& 59.0 &\underline{37.0} &\underline{41.3} & 27.9& 36.7& 29.3& 34.6 & 16.1& 25.9 &32.9 &40.4\\
Search-R1-instruct           &32.2 &42.0 &\underline{52.4} &\underline{60.3} &35.7 &41.2 &30.3 &39.6 &32.2 &38.0 &25.0 &36.9 &34.6 &43.0 \\
StepSearch-base         &30.0 &39.9 &47.3 &55.0 &32.2 &37.1 &32.1 &42.6 &\underline{37.1} &\underline{42.8} &33.0 &\underline{41.9} &35.3 &43.2\\
StepSearch-instruct         &33.9 &43.5 &51.1 &59.3 &34.9 &40.2 &\underline{33.2} &\underline{44.2} &34.7 &41.5 &\textbf{33.9} &\textbf{44.7} &\underline{37.0} &\underline{45.6} \\
HIPRAG-base              &11.0 &20.2 &23.4 &34.1 &14.9 &23.0 &10.3 &19.1 &8.30 &16.2 &10.5 &16.8 &13.1 &21.6\\
HIPRAG-instruct              &3.20 &9.50 &14.5 &24.2 &6.60 &13.7 &10.1 &18.4 &8.70 &18.6 &4.00 &11.9 &7.85 &16.1\\
\rowcolor{yellow!15}
AutoSearch     &\textbf{43.7} &\textbf{52.2} &\textbf{61.7} &\textbf{69.0} &\textbf{46.0} &\textbf{50.1} &\textbf{39.4} &\textbf{50.5} &\textbf{41.6} &\textbf{47.7} &\underline{33.1} &\textbf{44.7} &\textbf{44.3} &\textbf{52.4}\\
% AutoSearch(GRPO)    &\textbf{45.7} &\textbf{54.3} &\textbf{62.5} &\textbf{69.6} &44.5 &48.4 &\textbf{39.8} &\textbf{50.5} &39.6 &46.1 &\textbf{16.8} &24.9 &\textbf{34.7} &\textbf{46.1} \\

\midrule
\multicolumn{1}{c}{} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} \\

Search-R1-base           &\underline{1.23} &\underline{29.4} &\underline{1.29} &\underline{39.9} &\underline{1.35} &\underline{27.4} &1.63 &\underline{17.2} &1.95 &15.0 &\underline{1.69} &9.50 &1.52 &\underline{23.1} \\
Search-R1-instruct           &1.76 &18.3 &1.62 &32.3 &1.72 &20.7 &2.09 &14.5 &2.29 &14.1 &1.98 &12.6 &1.91 &18.8 \\
StepSearch-base         &2.95 &10.2 &2.90 &16.3 &2.94 &10.9 &3.19 &10.1 &3.51 &10.6 &3.03 &10.9 &3.09 &11.5\\
StepSearch-instruct         &1.46 &23.3 &1.57 &32.7 &1.45 &24.1 &2.05 &16.2 &2.29 &\underline{15.1} &2.07 &\underline{16.4} &1.82 &21.3\\
HIPRAG-base              &1.59 &6.92 &1.60 &14.6 &1.68 &8.88 &1.66 &6.22 &\underline{1.70} &4.87 &1.72 &6.11 &1.66 &7.93\\
HIPRAG-instruct              &1.28 &2.50 &1.32 &11.0 &\underline{1.35} &4.88 &\underline{1.58} &6.40 &1.84 &4.74 &\textbf{1.56} &2.57 &\underline{1.49} &5.35\\
\rowcolor{yellow!15}
AutoSearch     &\textbf{1.03} &\textbf{42.4} &\textbf{1.05} &\textbf{58.7} &\textbf{1.07} &\textbf{42.9} &\textbf{1.49} &\textbf{26.5} &\textbf{1.69} &\textbf{24.7} &1.83 &\textbf{18.1} &\textbf{1.36} &\textbf{35.6}\\
% AutoSearch(GRPO)    &\textbf{1.03} &\textbf{44.4} &\textbf{1.04} &\textbf{59.9} &1.08 &41.2 &\textbf{1.41} &\textbf{28.2} &\textbf{1.62} &24.5 &1.95 &\textbf{8.61} &1.61 &\textbf{21.5} \\

\midrule



% === Qwen2.5-7B Results ===
\rowcolor{green!10}
\multicolumn{15}{l}{\textit{\textbf{Base model: Qwen2.5-7b-Base/Instruct}}} \\

\multicolumn{1}{c}{} &
\makecell{\scriptsize \textbf{EM $\uparrow$}} &
\makecell{\scriptsize \textbf{F1 $\uparrow$}} &
\makecell{\scriptsize \textbf{EM $\uparrow$}} &
\makecell{\scriptsize \textbf{F1 $\uparrow$}} &
\makecell{\scriptsize \textbf{EM $\uparrow$}} &
\makecell{\scriptsize \textbf{F1 $\uparrow$}} &
\makecell{\scriptsize \textbf{EM $\uparrow$}} &
\makecell{\scriptsize \textbf{F1 $\uparrow$}} &
\makecell{\scriptsize \textbf{EM $\uparrow$}} &
\makecell{\scriptsize \textbf{F1 $\uparrow$}} &
\makecell{\scriptsize \textbf{EM $\uparrow$}} &
\makecell{\scriptsize \textbf{F1 $\uparrow$}} &
\makecell{\scriptsize \textbf{EM $\uparrow$}} &
\makecell{\scriptsize \textbf{F1 $\uparrow$}} \\


Search-R1-base          &\textbf{47.6} &\textbf{56.3} &\underline{63.7} &\underline{71.4} &\underline{45.7} &\underline{49.8} &\textbf{43.7} &\textbf{55.4} &38.7 &44.8 &41.1 &\underline{53.4} &\underline{46.8} &\underline{55.2}\\
Search-R1-instruct           &\underline{40.2} &48.5 &61.0 &68.4 &40.5 &45.4 &38.7 &49.0 &32.5 &38.1 &37.1 &49.6 &41.7 &49.8\\
StepSearch-base         &37.7 &47.9 &54.7 &63.3 &38.6 &44.0 &37.0 &48.6 &\underline{40.9} &\underline{47.3} &\textbf{42.7} &51.9 &41.9 &50.5\\
StepSearch-instruct         &34.2 &44.5 &51.6 &59.9 &34.9 &40.1 &38.9 &50.4 &39.8 &46.3 &40.3 &52.4 &40.0 &48.9\\
HIPRAG-instruct              &30.6 &42.0 &55.8 &65.2 &34.2 &42.4 &30.5 &42.7 &29.8 &38.3 &34.7 &47.8 &35.9 &46.4\\
\rowcolor{yellow!15}
% AutoSearch    &474 &560 &645 &721 &463 &503 &413 &530 &426 &492 &419 &514 & & \\
AutoSearch    &\textbf{47.6} &\underline{56.0} &\textbf{65.8} &\textbf{73.1} &\textbf{46.3} &\textbf{50.3} &\underline{42.7} &\underline{54.2} &\textbf{43.6} &\textbf{50.3} &\underline{41.9} &\textbf{54.9} &\textbf{48.0} &\textbf{56.5}\\
% AutoSearch(GRPO)    & & & & & & & & & & & & & & \\

\midrule
\multicolumn{1}{c}{} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} &
\makecell{\scriptsize \textbf{SD $\downarrow$}} &
\makecell{\scriptsize \textbf{SE $\uparrow$}} \\

Search-R1-base           &1.98 &24.0 &1.86 &34.2 &1.95 &23.4 &2.65 &16.5 &3.15 &12.3 &2.56 &16.1 &2.36 &21.1\\
Search-R1-instruct           &1.95 &20.7 &1.74 &35.0 &1.79 &22.6 &2.43 &15.9 &3.08 &10.5 &2.42 &15.3 &2.24 &20.0\\
StepSearch-base         &1.68 &22.4 &1.73 &31.6 &1.57 &24.7 &2.07 &17.8 &2.29 &\underline{17.9} &2.07 &20.7 &1.90 &22.5\\
StepSearch-instruct         &1.94 &17.6 &1.99 &25.9 &1.98 &17.6 &2.10 &18.6 &2.46 &16.2 &2.02 &19.9 &2.08 &19.3\\
HIPRAG-instruct              &\underline{1.07} &\underline{28.5} &\textbf{0.97} &\underline{57.8} &\underline{1.16} &\underline{29.5} &\underline{1.55} &\underline{19.7} &\underline{2.15} &13.8 &\textbf{1.45} &\underline{23.9} &\underline{1.39} &\underline{28.9}\\
\rowcolor{yellow!15}
% AutoSearch     &\textbf{1.07} &\textbf{44.5} &\underline{1.03} &\textbf{62.6} &\textbf{1.10} &\textbf{41.1} &\textbf{1.44} &\textbf{29.6} &\textbf{1.75} &\textbf{23.7} &\underline{1.74} &\underline{20.8} & &\\
AutoSearch    &\textbf{1.05} &\textbf{45.3} &\underline{1.04} &\textbf{63.3} &\textbf{1.09} &\textbf{40.8} &\textbf{1.34} &\textbf{31.2} &\textbf{1.58} &\textbf{25.9} &\underline{1.53} &\textbf{27.4} &\textbf{1.27} &\textbf{39.0} \\

\bottomrule
\end{tabular}
% } % end resizebox
\end{table*}
